Two-sided Facility Location

Recent years have witnessed the rise of many successful e-commerce marketplace platforms like the Amazon marketplace, AirBnB, Uber/Lyft, and Upwork, where a central platform mediates economic transactions between buyers and sellers. Motivated by these platforms, we formulate a set of facility location problems that we term Two-sided Facility location. In our model, agents arrive at nodes in an underlying metric space, where the metric distance between any buyer and seller captures the quality of the corresponding match. The platform posts prices and wages at the nodes, and opens a set of facilities to route the agents to. The agents at any facility are assumed to be matched. The platform ensures high match quality by imposing a distance constraint between a node and the facilities it is routed to. It ensures high service availability by ensuring flow to the facility is at least a pre-specified lower bound. Subject to these constraints, the goal of the platform is to maximize the social surplus (or gains from trade) subject to weak budget balance, i.e., profit being non-negative. We present an approximation algorithm for this problem that yields a $(1 + \epsilon)$ approximation to surplus for any constant $\epsilon > 0$, while relaxing the match quality (i.e., maximum distance of any match) by a constant factor. We use an LP rounding framework that easily extends to other objectives such as maximizing volume of trade or profit. We justify our models by considering a dynamic marketplace setting where agents arrive according to a stochastic process and have finite patience (or deadlines) for being matched. We perform queueing analysis to show that for policies that route agents to facilities and match them, ensuring a low abandonment probability of agents reduces to ensuring sufficient flow arrives at each facility.

==> obliviousProof.tex <==

\section{Proof of Theorem~\ref{thm:oblivious}}
\label{app:oblivious}
The rounding scheme proceeds in two steps. In the first step, we focus on the $y_i$ variables and make them integer without violating any of the constraints. This step relaxes the distance bound from $R$ to $4R$. 
We then show that the resulting solution can be modified to assign only one price and wage per node and deadline pair, again without violating any constraints.

\subsection{Structural Characterization: Proof of Lemma~\ref{lem:struct0}}
\label{app:struct}
We first formally prove the structural characterization stated in Lemma~\ref{lem:struct0}, that implies that in the neighborhood of any partially open virtual market, there is some demand/supply node that is (integrally) not an outlier. 

We first simplify the LP. Let $\Q_j' = \Q_j \setminus \{0\}$ and $\R_j' = \R_j \setminus \{0\}$. Let  $\eta_j = \sum_{q \in \Q_j'} \alpha_{jq}$ and  $\phi_j = \sum_{r \in \R_j'} \beta_{jr}$ respectively denote the fractions to which $j$ is assigned prices (wages) that correspond to non-zero demand (supply). We can rewrite the constraints (\ref{eq:single}) and (\ref{eq:singleprime}) as:
\begin{equation}
%\label{eq:single2} 
\label{eq:single3} 
\eta_j   =   \sum_{q \in \Q_j'} \sum_{i \in B_R(j)}  z_{ijq}  \le   1 \qquad \mbox{and} \qquad \phi_j  =   \sum_{r \in \R_j'} \sum_{i \in B_R(j)}  z_{ijr}   \le  1 \qquad  \forall j \in V 
% \qquad \forall j \in V 
\end{equation}
and set $\alpha_{j0} = 1 - \eta_j$, and $\beta_{j0} = 1 - \phi_j$.  Recall from Equations~(\ref{eq:welfare}) and~(\ref{eq:revone}) that $W_i$ and $R_i$ are respectively the welfare and profit of market $i$ in the LP optimum. %The LP optimum is $\sum_{i \in \F} W_i$, and the weak budget balance constraint implies $\sum_{i \in \F} R_i \ge 0$.

\medskip
We call node $j$ {\em fully demand-utilized} if $\eta_j = 1$, and {\em fully supply-utilized} if  $\phi_j = 1$. We say that node $j$ is {\em partially demand-connected} to market $i \in \F$ if $\sum_{q \in \Q_j'} z_{ijq} > 0$, and {\em partially supply-connected} if $\sum_{r \in \R_j'} z_{ijr} > 0$. Let $J_D(i)$ denote the set of nodes that are partially demand-connected to $i \in \F$, and $J_S(i)$ be the set that is partially supply-connected.  


\begin{lemma}
\label{lem:struct2}
\label{lem:struct}
In the LP optimum, for any $i \in \F$ with $y_i > 0$, we have $W_i > 0$. Furthermore, all except one market with $y_i > 0$ satisfy the following condition:  either $y_i = 1$; or there exists $j \in J_D(i)$, such that $j$ is {\em fully demand-utilized}; or there exists $j \in J_S(i)$ such that $j$ is {\em fully supply-utilized}.
\end{lemma}
\begin{proof}
First, note that $W_i \ge R_i$. %an elementary calculation shows that social surplus is at least the profit of a market, {\em i.e.}, $W_i \ge R_i$ for all $i$. To see this, note that for any $q,r$, we have $\V_j(q) \ge d_j q F_j^{-1}(q)$, and $\C_j(r) \le s_j r H_j^{-1}(r)$ if we integrate the expressions in Equation~(\ref{eq:valuation})  by parts. 
Suppose an open market has $W_i \le 0$. This implies $R_i \le 0$. Consider a different solution that sets $y_i = 0$ and $z_{ijq} = z_{ijr} = 0$ for all $j \in V, q \in \Q_j', r \in \R_j'$. We adjust $\eta_j$ and $\phi_j$ for each $j \in V$ to preserve constraint (\ref{eq:single3}). This new solution has $W_i = R_i = 0$ and has at least as large surplus and profit. Since we set all LP variables corresponding to $i$ to zero, this satisfies constraints (\ref{eq:open0}), (\ref{eq:flowbalance0}), and (\ref{eq:lowerbound0}), and is therefore feasible for the LP.

\medskip
We therefore only focus on markets whose $W_i > 0$. Consider the set of these markets and split them into two groups. Let 
$$S_1 = \{ i \in \F \ | y_i \in (0,1) \mbox{ and } R_i < 0\} \qquad \mbox{and} \qquad S_2 = \{ i \in \F \ | y_i \in (0,1) \mbox{ and } R_i \ge 0\}$$
Assume that for all of these markets, there is no $j \in J_D(i)$, such that $j$ is {\em fully demand-utilized} and no $j \in J_S(i)$ such that $j$ is {\em fully supply-utilized}

First consider the markets in set $S_2$, we can increase the LP variables till the condition of the lemma is satisfied; this process only increases both profit and welfare, preserving all constraints. We do this as follows: Suppose no $j  \in J_D(i)$  is fully demand-utilized and no $j \in J_S(i)$ is fully supply-utilized. In this case, let 
$$ \theta = \min\left( \frac{1}{y_i}, \min_{j \in J_D(i)} \left( \frac{1 -  \sum_{q \in \Q_j'} \sum_{i' \neq i}  z_{i'jq}}{\sum_{q \in \Q_j'}  z_{ijq} }\right), \min_{j \in J_S(i)} \left( \frac{1 -  \sum_{r \in \R_j'} \sum_{i' \neq i}  z_{i'jr}}{\sum_{r \in \R_j'}  z_{ijr} } \right) \right)$$  
Since $\eta_j < 1$ for all $j \in J_D(i)$ and $\phi_j < 1$ for all $j \in J_S(i)$, we have $\theta > 1$. Suppose we increase $y_i$, $z_{ijq}$ for all $j \in J_D(i), q \in \Q_j'$, and $z_{ijr}$ for all $j \in J_S(i)$, $r \in \R_j'$ by a factor of $\theta$. We will still have $\eta_j \le 1$ for all $j \in J_D(i)$ and $\phi_j \le 1$ for all $j \in J_S(i)$. However, either $y_i$ or one of these values will become exactly $1$. Note that since we scaled all LP variables corresponding to $i$ by the same factor, this preserves constraints (\ref{eq:open0}), (\ref{eq:flowbalance0}), and (\ref{eq:lowerbound0}). The surplus and profit of this market increase by a factor $\theta > 1$, which contradicts the optimality of the LP solution. Therefore, the markets in $S_2$ all have a neighboring $j$ that is either fully demand-utilized or fully supply-utilized.

Next consider the markets in set $S_1$. Suppose the condition in the lemma is not satisfied, so that there are two markets $i$ and $i'$ with $y_i, y_{i'}  \in (0,1)$, and with no neighboring $j$ that is either fully demand-utilized or fully supply-utilized. Suppose $W_i/|R_i| = a$ and $W_{i'}/|R_{i'}|= b$ with $a \ge b$. We multiply each LP variable corresponding to $i$ by a factor of $(1+\delta)$, and multiply each LP variable corresponding to $i'$ by a factor of $\left(1 - \frac{W_{i}}{W_{i'}}  \delta\right)$. Using the same argument as above, this process preserves the constraints that are specific to a market, since all variables are changed by the same factor.  The increase in welfare of market $i$ is $\delta W_i$, and the decrease in welfare of market $i'$ is $\delta W_i$, so the overall welfare is preserved. The decrease in profit of market $i$ is $|R_i| \delta$, and the increase in profit of market $i'$ is $|R_{i'}| \frac{W_{i}}{W_{i'}}  \delta \ge |R_i| \delta$ by our assumption that $a \ge b$. Therefore, this process cannot decrease profit, hence all constraints are preserved. We choose $\delta$ as the smallest value that either makes market $i$ have $y_i = 1$ or one neighboring $j$ either fully supply or demand utilized, or that sets the variables of market $i'$ to zero. In all cases, the size of set $S_1$ reduces by one. We repeat this process till there is only one market in $S_1$, completing the proof.
\end{proof}
 
\begin{corollary}
\label{cor1}
There is a $(1+\epsilon)$-approximation to the LP optimum where any market with $y_i > 0$ satisfies the following condition:  either $y_i = 1$; or there exists $j \in J_D(i)$, such that $j$ is {\em fully demand-utilized}; or there exists $j \in J_S(i)$ such that $j$ is {\em fully supply-utilized}.
\end{corollary}
\begin{proof}
By Constraint~(\ref{eq:tighter2}), there is a set of markets $S$ that are fully open ({\em i.e.}, $y_{i} = 1$) and $\sum_{i \in S} W_{i} \ge \W \frac{1-\epsilon}{\epsilon}$ by Constraint~(\ref{eq:tighter3}). The rounding in Lemma~\ref{lem:struct2} does not touch these markets, since we only increase/decrease variables corresponding to partially open markets ({\em i.e.}, those with $y_i \in (0,1)$). Lemma~\ref{lem:struct2} implies there is only market $i$ that violates the condition of the corollary. This market must have welfare $W_i \le \W y_i \le \W$ by Constraint~(\ref{eq:tighter1}).  This means closing this market (setting all its associated variables to zero) reduces the LP optimum by at most a factor of $(1-\epsilon)$. Since the previous lemma implies this market had $R_i  < 0$, this means closing it only increases profit, preserving weak budget balance.
\end{proof}



%In our rounding scheme, we make $y_i$ variables integer without violating any of the constraints. This step relaxes the distance bound from $R$ to $4R$. Therefore, $B_R$ is replaced by $B_{4R}$ in the LP during the rounding process. 

\subsection{Rounding Virtual Markets}
\label{app:round}
Initially, all virtual markets $i \in \F$ with $y_i > 0$ are {\em partially open}. Node $j \in V$ is {\em untouched} if for all $i$ such that $j \in J_D(i) \cup J_S(i)$, the market $i$ is partially open.  Let $U$ be the set of {\em untouched} nodes, and let $Z$ be the set that is either fully demand-utilized or fully supply-utilized.  Let $U_f = U \cap Z$. 

\medskip
\noindent {\bf Phase 1.} Consider any $j \in U_f$. W.l.o.g., assume $\eta_j = 1$; the case where $\phi_j = 1$ is symmetric.  Let  $ N(j) = \{i | j \in J_D(i) \}$.  For every $i \in N(j)$, we ``move" $i$ to location $j$; call the new virtual market at location $j$ as $i^*$. This means we set
%I said new because otherwise we need an extre neq i* and also the definition of touched won't be the same with reassigned in the previous step exactly 
\begin{itemize}
\item $\bar{y}_{i^*} \leftarrow \sum_{i \in N(j)} y_i$ and $\bar{y}_i \leftarrow 0 \qquad \forall i \in N(j)$;
\item $\bar{z}_{i^*j'q} \leftarrow \sum_{i \in N(j)} z_{ij'q}$  and $\bar{z}_{ij'q} \leftarrow 0 \qquad \forall j' \in V, q \in \Q_{j'}, i \in N(j)$
\item $\bar{z}_{i^*j'r} \leftarrow \sum_{i \in N(j)} z_{ij'r}$  and $\bar{z}_{ij'r} \leftarrow 0 \qquad \forall j' \in V,  r \in \R_{j'}, i \in N(j)$
\end{itemize}

From constraint (\ref{eq:open0}), and the fact that $\eta_j = 1$, we have:  
$$\bar{y}_{i^*}  =  \sum_{i  \in N(j)}  y_i \ge \sum_{i \in B_R(j)} \sum_{q \in \Q_j'} z_{ijq} = \eta_j = 1$$ 
Subsequently, we mark every $i \in N(j)$  as {\em closed}, and mark $i^*$ as {\em completely open}. Furthermore, we mark every $j'$ that was reassigned in the above steps as {\em touched}.

Note that in the last three steps, any agents at a node $j'$ that was initially assigned to $i \in N(j)$ is now assigned to $i^*$. Since  each of the distances $j' \rightarrow i$ and $i \rightarrow j$ is at most $R$, the distance from $j'$ to $i^*$ is at most $2R$. Therefore, this step relaxes the distance of a feasible assignment to a virtual market from $R$ to $2R$.

This process trivially preserves the objective and weak budget balance, as well as constraints (\ref{eq:single3}). Moreover, constraints  (\ref{eq:open0}) and (\ref{eq:flowbalance0}) are satisfied since we add both sides of the constraints corresponding to $i \in N(j)$ to obtain the constraint for $i^*$. Finally, to see that (\ref{eq:lowerbound0}) is satisfied for $i^*$, note that 
$$ \sum_{j' \in J_D(i^*)}   \sum_{q \in \Q_{j'}'}  d_{j'} q \bar{z}_{i^*j'q}   =  \sum_{i \in N(j)} \sum_{j' \in J_D(i)} \sum_{q \in \Q_{j'}'} d_{j'}  q z_{ij'q}  \ge  \L \sum_{i \in N(j)} y_i  \ge   \L
$$
    
We continue this process, finding a node $j \in U_f$, and merging all virtual markets in $N(j)$ to one location. At the end of this process, the set $U_f$ is empty. 

\medskip
\noindent {\bf Phase 2.} At the end of Phase 1, each node $j$ which is {\em touched } (including all {\em fully utilized} nodes) route some fraction of their demand (or supply) to at least one virtual market that is completely open. However, there could still be partially open markets with $y_i \in (0,1)$ to which demand and supply are assigned. Consider these partially open markets in arbitrary order. Suppose we are considering market $i$ and there exists {\em touched} and {\em fully utilized} node $j$ such that $\sum_{q \in \Q_j'} z_{ijq} > 0$ (resp. $\sum_{r \in \R_j'} z_{ijr} > 0$).  Consider the completely open market $i^*$ such that $\sum_{q \in \Q'_j} \bar{z}_{i^*jq} > 0$ or $\sum_{r \in \R'_j} \bar{z}_{i^*jr} > 0$. We move the virtual market $i$ to location $i^*$, updating the variables just as in Phase 1; {\em i.e.}, we set
\begin{itemize}
\item $\bar{y}_{i^*} \leftarrow \bar{y}_{i^*} +  y_i$ and $\bar{y}_i \leftarrow 0$;
\item $\bar{z}_{i^*j'q} \leftarrow \bar{z}_{i^*j'q} + z_{ij'q}$  and $\bar{z}_{ij'q} \leftarrow 0 \qquad \forall j' \in V, q \in \Q_{j'}$
\item $\bar{z}_{i^*j'r} \leftarrow \bar{z}_{i^*j'r} + z_{ij'r}$  and $\bar{z}_{ij'r} \leftarrow 0 \qquad \forall j' \in V,  r \in \R_{j'}$
\end{itemize}

The argument that all constraints are preserved follows just as before. For any $j'$ that was partially assigned to $i$, the new assignment is to $i^*$. This distance is at most 
$$c(j',i^*) \le c(j',i) + c(i,j) + c(j,i^*) \le R + R + 2R = 4R$$
 where we note that the distance $j \rightarrow i^*$ was at most $2R$ because $j$ was potentially reassigned to $i^*$ in Phase 1.  We mark all nodes $j'$ that are reassigned in this process as {\em touched}.

\medskip
At the end of this process, suppose there are still partially open markets with $y_i \in (0,1)$. By Corollary~\ref{cor1}, each of these markets $i$ must have some $j \in Z$ partially assigned to it. At the end of Phase 1, we have the invariant that $j \notin U_f$, since $U_f$ is empty. This means $j$ was touched on Phase 1. But in that case, $i$ must have been reassigned in Phase 2, which is a contradiction.  Therefore, at this point, all virtual markets are either closed ($\bar{y}_i = 0$) or completely open ($\bar{y}_i \ge 1$). Furthermore, for any variable $\bar{z}_{ijq} > 0$ (resp. $\bar{z}_{ijr} > 0$), the virtual market $i$ is completely open; the distance from $j$ to $i$ is at most $4R$; for each completely open market, the rate of supply equals the rate of demand (Constraint (\ref{eq:flowbalance0})), and finally, the total flow is at least $\L$ (Constraint (\ref{eq:lowerbound0})).  

\subsection{Rounding Prices and Wages}
The rounding the $\alpha_{jq}, \beta_{jr}$ variables  to integer values now follows from Lemma~\ref{lem:increase}. In summary, the price at node $j$ is $F_j^{-1}(\hat{q}_j)$ and the wage at $j$ is $H_j^{-1}(\hat{r}_j)$. An arriving demand (resp. supply) agent at node $j$ is routed to market $i$ with probability $\hat{z}_{ij\hat{q}_j}$ (resp. $\hat{z}_{ij\hat{r}_j}$).  This yields theorem~\ref{thm:oblivious}.


